Cluster detection in weak lensing surveys

We present an efficient and robust approach for extracting clusters of galaxies from weak lensing survey data and measuring their properties. We use simple, physically-motivated cluster models appropriate for such sparse, noisy data, and incorporate our knowledge of the cluster mass function to optimise the detection of low-mass objects. Despite the method's non-linear nature, we are able to search at a rate of approximately half a square degree per hour on a single processor, making this technique a viable candidate for future wide-field surveys. We quantify, for two simulated data-sets, the accuracy of recovered cluster parameters, and discuss the completeness and purity of our shear-selected cluster catalogues.

==> additional.tex <==

In order to demonstrate our algorithm we use simulated weak lensing maps made 
from ray tracing through N-body simulations of structure formation
(\citet{white05}), covering $3 \times 3$ degree field of view. The cosmological 
model is taken to be a concordance $\Lambda$CDM model with parameters 
$\Omega_m=0.3$, $\Omega_{\Lambda}=0.8$, $\sigma_8=0.9$ and the Hubble parameter 
$h=0.7$. The simulations emplyed $384^3$ equal mass ($10^{10} M_{\sun} h^{-1}$) 
dark matter particles in a periodic cubical box of side $200 h^{-1} Mpc$ run
to $z=0$. The source redshift distribution was taken to be: 
\begin{equation}
p(z) \sim z^2 e^{-(z/z_0)^b}
\end{equation}
with $z_0=1.0$ and $b=1.5$.

The halo catalogue contains $563$ halos with $M_{200} > 5 \times 10^{13} 
h^{-1} M_{\sun}$ and redshifts between $0.0$ and $2.7$.

There are roughly $200$ galaxies per square arcminute in the simulation which
represents the deepest space-based surveys. In practice the signal-to-noise 
magnitude threshold gives around $100$ galaxies per square arcminute and then 
insisting on knowing the photo-z of each source pushes the number down to 
$40-70$ galaxies per square arcminute. Since there is no colour/magnitude
information for the sources available in these simulations, we pick $65$ 
galaxies per square arcminute randomly from the source catalogue. The intrinsic
ellipticity distribution of the source galaxies is assumed to be Gaussian with  
$\sigma_{int}=0.25$. We add Gaussian observational noise with standard 
deviation $\sigma_{obs}=0.20$ to the sheared ellipticity of each galaxy.

Modelling the whole $3 \times 3$ degree$^2$ field of view represents a highly
computationally expensive task and the MultiNest algorithm would require a
prohibitely large no. of live points to detect clusters with enough resolution.
We therefore divide the data in $16$ patches of $0.75 \times 0.75$ degree$^2$
each and use $3000$ live points to model each one of these $16$ patches. As
before, we expand the ranges of uniform priors on the position of cluster 
centers to allow them to lie a little outside their respective patches.



